Efficient delay-tolerant particle filtering

This paper proposes a novel framework for delay-tolerant particle filtering that is computationally efficient and has limited memory requirements. Within this framework the informativeness of a delayed (out-of-sequence) measurement (OOSM) is estimated using a lightweight procedure and uninformative measurements are immediately discarded. The framework requires the identification of a threshold that separates informative from uninformative; this threshold selection task is formulated as a constrained optimization problem, where the goal is to minimize tracking error whilst controlling the computational requirements. We develop an algorithm that provides an approximate solution for the optimization problem. Simulation experiments provide an example where the proposed framework processes less than 40% of all OOSMs with only a small reduction in tracking accuracy.

==> section5.tex <==
\section{Asymptotic Optimality of the Proposed Algorithm} \label{Sec:5}

In this section we will consider the conditions under which the
unconditional measurement independence assumption made in the
previous section for the Gaussian approximation is expected to hold.
The assumption is made to simplify the algorithm derivation and
reduce computational requirements of the algorithm, leading to the
sub-optimality of the derived constrained MSE minimization
algorithm. However, when the independence assumption holds exactly,
the proposed algorithm becomes optimal with respect to minimizing
the MSE calculated from the employed Gaussian approximation. The
conditions established in this section help us understand when the
performance of the proposed sub-optimal algorithm is expected to
approach that of the optimal OOSM selection algorithm based on the
minimization of the MSE calculated from the employed Gaussian
approximation of posterior.


In order to investigate the optimality conditions, we need
expressions for the unconditional (unconditional on the state value,
recall that conditioning on $\widetilde{\mathcal{W}}_{1:k,k}$ is
implied unless stated otherwise) measurement cross-covariance. Using
the independence of measurement and diffusion noises from each other
and from the state and independence of $\zeta_{m}^{s}$ and
$\zeta_{n}^{j}$ for any $m\neq n$ or $s\neq j$, we have for $m>n$
and any $s,j$:
\begin{align} \label{eqn:meas_cross_cov}
\bR_{Y_{m}^{s} Y_{n}^{j} } &= \bE\{ (Y_{m}^{s}-\bE\{ Y_{m}^{s}
\})(Y_{n}^{j}-\bE\{
Y_{n}^{j} \})^T  \} \\
&= \bE\{ (\bH_{m}^{s}(\bF_{m,n}(X_{n} - \mu_{X_{n}}) +
\sum_{j=n+1}^m \bF_{m,j} \upsilon_{j}) + \zeta_{m}^{s})
(\bH_{n}^{j}(X_{n} - \mu_{X_{n}})
+ \zeta_{n}^{j})^T \} \\
&= \bH_{m}^{s}\bF_{m,n}\bE\{ (X_{n} - \mu_{X_{n}})(X_{n} -
\mu_{X_{n}})^T\}{\bH_{n}^{j}}^T
\\
&+ \bH_{m}^{s}\bF_{m,n}\bE\{ (X_{n} -
\mu_{X_{n}}){\zeta_{n}^{j}}^T\}
\\
&+ \sum_{j=n+1}^m \bF_{m,j} \bE\{ \upsilon_{j}(X_{n} -
\mu_{X_{n}})^T\}{\bH_{n}^{j}}^T \\
&+ \sum_{j=n+1}^m \bF_{m,j} \bE\{ \upsilon_{j}{\zeta_{n}^{j}}^T\} +
\bE\{ \zeta_{m}^{s}(X_{n} -
\mu_{X_{n}})^T \}\bH_{n}^{j} + \bE\{ \zeta_{m}^{s} {\zeta_{n}^{j}}^T \}  \\
&= \bH_{m}^{s} \bF_{m,n} \bR_{X_{n} X_{n}} {\bH_{n}^{j}}^T
\end{align}
Note that for $m<n$ $\bR_{Y_{m}^{s} Y_{n}^{j} } = \bR_{Y_{n}^{s}
Y_{m}^{j} }^T = \bH_{m}^{s} \bR_{X_{m} X_{m}} \bF_{n,m}^T
{\bH_{n}^{j}}^T$.

We are now ready to state our main result in this section.

\begin{theorem} \label{th:asymptotic_optimality}
Let $\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}$, $\bR_{X_{k}
\mathcal{Z}_{k}}$ be defined
via~\eqref{eqn:meas_cov},~\eqref{eqn:meas_state_cross-cov}
and~\eqref{eqn:meas_cross_cov} and let $\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}$ be the block-diagonal matrix whose blocks are
defined via~\eqref{eqn:meas_cov} and organized to match those of
$\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}$. Suppose that the following
assumptions hold:
\begin{itemize}
\item[$\mathcal{A}_1$:] $\rho(\bR_{X_{n} X_{n}}) <
\infty$, $\forall k-\ell \leq n < k$
\item[$\mathcal{A}_2$:] $\rho(\bH_{m}^{s} {\bH_{m}^{s}}^T)^{1/2} < \infty$ and $\rho({\bH_{m}^{s}}^T \bH_{m}^{s})^{1/2} < \infty$, $\forall k-\ell \leq m
< k$ and $\forall s \in \mathcal{V}_m$
\item[$\mathcal{A}_3$:] $\rho(\bF_{m,n} \bF_{m,n}^T)^{1/2} < \infty$, $\forall k-\ell\leq n\leq m$ and $k-\ell \leq m \leq k$
\end{itemize}

Then we have for any $\ell,K < \infty$, $\mathcal{Z}_{k}$ and $k>1$:
\begin{align}
\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})
\rightarrow \infty \Rightarrow | \tr \bR_{X_{k}
\mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}\bR_{\mathcal{Z}_{k} X_{k}} -  \tr \bR_{X_{k}
\mathcal{Z}_{k}}\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}\bR_{\mathcal{Z}_{k} X_{k}} | \rightarrow 0,
\end{align}
where $\lambda_{\min}(\cdot) = \min_{i}\lambda_i(\cdot)$
\end{theorem}

\begin{proof}
Since $\tr(\cdot) = \sum_i \lambda_i(\cdot)$ we have
\begin{align} \label{eqn:technical_0}
| \tr \bR_{X_{k} \mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}\bR_{\mathcal{Z}_{k} X_{k}} &-  \tr \bR_{X_{k}
\mathcal{Z}_{k}}\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}\bR_{\mathcal{Z}_{k} X_{k}} |\\
 &= | \tr
\bR_{X_{k} \mathcal{Z}_{k}}(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\bR_{\mathcal{Z}_{k} X_{k}}| \\
&\leq K \ell \rho(\bR_{X_{k} \mathcal{Z}_{k}}(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\bR_{\mathcal{Z}_{k} X_{k}}),\\
&\leq K \ell \rho(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\rho(\bR_{X_{k}
\mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k} X_{k}}), \\
&\leq K \ell \lambda_{\min}^{-1}(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}})
\lambda_{\min}^{-1}(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}) \rho(
\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}) \rho(\bR_{X_{k}
\mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k} X_{k}}),\\
&\leq \frac{K\ell\rho(\bR_{X_{k} \mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k} X_{k}})
\rho( \bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}})}{(\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})
- \rho(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}-\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}))
\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})},
\end{align}
where $\rho(\cdot) = \max_i |\lambda_{i}(\cdot)|$ is the spectral
radius. Using the variational characterization of spectral radius we
have for a square matrix $\bA$ and an arbitrary real matrix $\bC$:
\begin{align}
\rho(\bC^T \bA \bC) &= \max_{\bx\neq 0}\frac{|\bx^T\bC^T \bA \bC
\bx|}{\bx^T\bx} = \max_{\bx\neq 0}\left(\frac{|\bx^T\bC^T \bA \bC
\bx|}{\bx^T\bC^T\bC\bx} \frac{\bx^T\bC^T\bC\bx}{\bx^T\bx}\right) \\
&\leq \max_{\bx\neq 0}\left( \max_{\by\neq 0}
\frac{|\by^T\bA\by|}{\by^T\by}
\frac{\bx^T\bC^T\bC\bx}{\bx^T\bx}\right) \\
&\leq \rho(\bA) \rho(\bC^T \bC),
\end{align}
resulting in:
\begin{align} \label{eqn:techncal_3}
\rho(\bR_{X_{k} \mathcal{Z}_{k}}(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\bR_{\mathcal{Z}_{k} X_{k}}) \leq
\rho(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\rho(\bR_{X_{k}
\mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k} X_{k}}).
\end{align}
Furthermore, using the decomposition
\begin{align}
\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1} = \bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}^{-1}(
\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}) \bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}^{-1}.
\end{align}
we conclude
\begin{align} \label{eqn:technical_4}
\rho(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}) &\leq \rho(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\rho( \bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} -
\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}) \rho(\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}) \\
&= \lambda_{\min}^{-1}(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}})
\lambda_{\min}^{-1}(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}) \rho(
\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}).
\end{align}
Since the eigenvalues of the block-diagonal matrix are the
eigenvalues of its blocks we have
$\lambda_{\min}(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}) =
\min_{s,m}\lambda_{\min}(\bR_{Y_{m}^{s}Y_{m}^{s}})$. Moreover,
taking into account that for any $\bA$ and $\bC$
$\lambda_{\min}(\bA+\bC) \geq \lambda_{\min}(\bA) +
\lambda_{\min}(\bC)$ and recalling~\eqref{eqn:meas_cov} we observe:
\begin{align}
\lambda_{\min}(\bR_{Y_{m}^{s}Y_{m}^{s}}) &=
\lambda_{\min}(\bH_{m}^{s} \bR_{X_{m} X_{m}} {\bH_{m}^{s}}^T +
\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}) \\
&\geq \lambda_{\min}(\bH_{m}^{s} \bR_{X_{m} X_{m}} {\bH_{m}^{s}}^T)
+
\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}) \\
&\geq \lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}).
\end{align}
The last inequality holds since $\bR_{X_{m} X_{m}}$ is a covariance
matrix and hence ${\bH_{m}^{s}} \bR_{X_{m} X_{m}} {\bH_{m}^{s}}^T$
is positive semidefinite. Similarly, since $\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}$ is a covariance matrix and as such is positive
semidefinite we deduce:
\begin{align} \label{eqn:technical_5}
\lambda_{\min}(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}) &=
\lambda_{\min}(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} +
(\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}})) \\
&\geq \max[0, \lambda_{\min}(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}})
+ \lambda_{\min}(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}-\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}})] \\
&\geq \max[0,
\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}) -
\rho(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}-\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}})]
\end{align}

To obtain upper bound on the latter spectral radius we use the
following observation for a square block matrix $\bA$ with blocks
$\bA_{i,j}$:
\begin{align} \label{eqn:rh_A_block}
\rho(\bA) \leq \sum_{i,j} \rho(\bA_{i,j}^T\bA_{i,j})^{1/2},
\end{align}
The proof of this fact is organized in a short lemma below.
\begin{lemma}
Let $\bA \in \mathbb{R}^{K\times K}$ be a block matrix consisting of
blocks $\bA_{i,j}\in \mathbb{R}^{K_i\times M_j}$ then the following
holds: $\rho(\bA) \leq \sum_{i,j} \rho(\bA_{i,j}^T\bA_{i,j})^{1/2}$
\end{lemma}
\begin{proof}
Let $\{\bx_{i}\}$ and $\{ \by_{j} \}$ be two partitionings of vector
$\bX \in \mathbb{R}^{K}$ such that $\bX^T = [\bx_{1}^T, \bx_{2}^T,
\ldots]$, $\bx_{i} \in \mathbb{R}^{K_i}, \forall i$ and $\bX^T =
[\by_{1}^T, \by_{2}^T, \ldots]$, $\by_{j} \in \mathbb{R}^{M_j},
\forall j$. Write the variational characterization of the spectral
radius and expand it in terms of blocks:
\begin{align} \label{eqn:rho_bA_decomp}
\rho(\bA) &= \max_{\bX \neq 0} \frac{|\bX^T \bA \bX|}{\bX^T \bX} \\
&= \max_{\bX \neq 0} \frac{|\sum_{i,j} \bx_i^T \bA_{i,j}
\by_{j}|}{\bX^T \bX} \\
&\leq \max_{\bX \neq 0} \frac{\sum_{i,j} |\bx_i^T \bA_{i,j}
\by_{j}|}{\bX^T \bX} \\
&\leq \sum_{i,j} \max_{\bX \neq 0} \frac{ |\bx_i^T \bA_{i,j}
\by_{j}|}{\bX^T \bX}.
\end{align}
Now, for every summand use the Cauchy-Schwarz inequality and take
into account the fact that $\bx_i^T \bx_i /\bX^T \bX \leq 1, \forall
i$:
\begin{align}
\max_{\bX \neq 0} \frac{ |\bx_i^T \bA_{i,j} \by_{j}|}{\bX^T \bX}
&\leq \max_{\bX \neq 0} \frac{ |\bx_i^T \bx_i|^{1/2}}{|\bX^T
\bX|^{1/2}} \frac{ |\by_{j}^T \bA_{i,j}^T \bA_{i,j}
\by_{j}|^{1/2}}{|\bX^T \bX|^{1/2}} \\
&\leq \max_{\bX \neq 0} \frac{ |\by_{j}^T \bA_{i,j}^T \bA_{i,j}
\by_{j}|^{1/2}}{|\bX^T \bX|^{1/2}}.
\end{align}
Similarly, note the fact that $\by_j^T \by_j \leq \bX^T \bX, \forall
j$:
\begin{align}
\max_{\bX \neq 0} \frac{ |\by_{j}^T \bA_{i,j}^T \bA_{i,j}
\by_{j}|^{1/2}}{|\bX^T \bX|^{1/2}} &\leq \max_{\bX \neq 0} \frac{
|\by_{j}^T \bA_{i,j}^T \bA_{i,j} \by_{j}|^{1/2}}{|\by_{j}^T
\by_{j}|^{1/2}} \\
&= \left( \max_{\by_{j} \neq 0} \frac{ |\by_{j}^T \bA_{i,j}^T
\bA_{i,j} \by_{j}|}{|\by_{j}^T \by_{j}|} \right)^{1/2}.
\end{align}
This is the variational characterization of $\rho(\bA_{i,j}^T
\bA_{i,j})^{1/2}$. Substituting it into~\eqref{eqn:rho_bA_decomp}
completes the proof.
\end{proof}


Noting that all diagonal blocks of $\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}-\bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}$ are null and
using~\eqref{eqn:rh_A_block} we have:
\begin{align} \label{eqn:technical_2}
\rho( \bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}) &\leq
\sum_{m=k-\ell}^{k-1}\sum_{s\in\mathcal{S}_{m,k}} \left(
\sum_{n=k-\ell, n\neq m}^{k-1} \sum_{j\in\mathcal{S}_{n,k}}
\rho(\bR_{Y_{m}^{s}Y_{n}^{j}} \bR_{Y_{n}^{j}Y_{m}^{s}})^{1/2} +
\sum_{j\in\mathcal{S}_{m,k},j\neq
s} \rho(\bR_{Y_{m}^{s}Y_{m}^{j}} \bR_{Y_{m}^{j}Y_{m}^{s}}) \right)^{1/2} \\
&\leq K\ell(K\ell-1) \max_{s,m} \max_{j\neq s \vee n\neq m}
\rho(\bR_{Y_{m}^{s}Y_{n}^{j}}
\bR_{Y_{n}^{j}Y_{m}^{s}})^{1/2} \\
&\leq K\ell(K\ell-1) \max_{s,m} \max_{j\neq s \vee n\neq m}
\max[\rho(\bH_{m}^{s} \bF_{m,n} \bR_{X_{n} X_{n}} {\bH_{n}^{j}}^T
{\bH_{n}^{j}} \bR_{X_{n}
X_{n}} \bF_{m,n}^T {\bH_{m}^{s}}^T)^{1/2} , \nonumber\\
& \rho(\bH_{n}^{j} \bF_{n,m} \bR_{X_{m} X_{m}} {\bH_{m}^{s}}^T
{\bH_{m}^{j}} \bR_{X_{m}
X_{m}} \bF_{n,m}^T {\bH_{n}^{j}}^T)^{1/2}] \\
&\leq K\ell(K\ell-1) \max_n \rho(\bR_{X_{n} X_{n}}) \max_{s,m}
\rho(\bH_{m}^{s} {\bH_{m}^{s}}^T)^{1/2} \max_{s,m}
\rho({\bH_{m}^{s}}^T \bH_{m}^{s})^{1/2}  \max_{n \leq m}
\rho(\bF_{m,n}\bF_{m,n}^T)^{1/2}
\end{align}
where in the last expression the maximum is over spectral radii of
all non-diagonal blocks.

Finally, observing that $\bR_{X_{k}
\mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k}X_{k}} = \sum_{s,m} \bR_{X_{k}
Y_{m}^{s}} \bR_{X_{k} Y_{m}^{s}}^T$ and
recalling~\eqref{eqn:meas_state_cross-cov}
\begin{align} \label{eqn:technical_1}
\rho(\bR_{X_{k} \mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k}X_{k}}) &\leq
\sum_{s,m} \rho(\bR_{X_{k} Y_{m}^{s}} \bR_{X_{k}
Y_{m}^{s}}^T) \\
&= \sum_{s,m} \rho(\bF_{k,m} \bR_{X_{m} X_{m}} {\bH_{m}^{s}}^T
{\bH_{m}^{s}} \bR_{X_{m} X_{m}}
\bF_{k,m}^T ) \\
&\leq K\ell \max_{s,m} \rho(\bF_{k,m} \bF_{k,m}^T)
\rho({\bH_{m}^{s}}^T {\bH_{m}^{s}}) \rho(\bR_{X_{m} X_{m}})^2.
\end{align}

Summarizing our results and invoking our assumptions we see
from~\eqref{eqn:technical_1} that $\rho(\bR_{X_{k}
\mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k}X_{k}}) < \infty$ and
from~\eqref{eqn:technical_2} that $\rho( \bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k} \mathcal{Z}_{k}}) < \infty$.
Thus for a sufficiently large
$\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})$ we can
write using~\eqref{eqn:techncal_3},~\eqref{eqn:technical_4}
and~\eqref{eqn:technical_5}:
\begin{align}
\rho(\bR_{X_{k} \mathcal{Z}_{k}}(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\bR_{\mathcal{Z}_{k} X_{k}}) \leq
\frac{\rho(\bR_{X_{k} \mathcal{Z}_{k}}\bR_{\mathcal{Z}_{k} X_{k}})
\rho( \bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}} - \bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}})}{(\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})
- \rho(\bB_{\mathcal{Z}_{k} \mathcal{Z}_{k}}-\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}))
\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})},
\end{align}
leading us to the conclusion that
$\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})
\rightarrow \infty \Rightarrow \rho(\bR_{X_{k}
\mathcal{Z}_{k}}(\bR_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1}-\bB_{\mathcal{Z}_{k}
\mathcal{Z}_{k}}^{-1})\bR_{\mathcal{Z}_{k} X_{k}}) \rightarrow 0$
and completing the proof taking into
account~\eqref{eqn:technical_0}.
\end{proof}


The implications of the theorem are the following. As the minimal
eigenvalues of the noise matrices for all sensors involved and at
all times go to infinity, the block-diagonal assumption employed to
derive the OOSM selection algorithm in the previous section holds
exactly, under certain regularity conditions.

The regularity conditions imposed by the
Theorem~\ref{th:asymptotic_optimality} are natural. Assumption
$\mathcal{A}_1$ requires extended Kalman smoother covariance
$\bR_{X_{n} X_{n}}$ to have finite spectral radius. Thus assumption
$\mathcal{A}_1$ basically requests the stability (including the
numerical stability) of the EKS. Assumption $\mathcal{A}_2$ and
$\mathcal{A}_3$ require the spectral radia of matrices $\bH_{m}^{s}
{\bH_{m}^{s}}^T$, ${\bH_{m}^{s}}^T \bH_{m}^{s}$ and $\bF_{m,n}
\bF_{m,n}^T$ to be finite. Thus these requirements are most
naturally related to the differentiability of measurement,
$h_{k}^{s}(\cdot)$, and state transition, $f_{k}(\cdot)$, mappings.
It is straightforward to see that if the measurement and transition
functions are differentiable (sufficiently smooth), leading to
$\bF_{m}$ and $\bH_{m}^{s}$ with finite elements (existence of
$\bF_{m}$ and $\bH_{m}^{s}$), assumptions $\mathcal{A}_2$ and
$\mathcal{A}_3$ hold by the Gershgorin disc theorem~[Horn and
Johnson]. Hence assumptions $\mathcal{A}_2$ and $\mathcal{A}_3$ do
not impose any additional constraints on the applicability of the
results of the theorem: any scenario when the EKS functions normally
and can be implemeted leads to the assumptions being satisfied.

The asymptotics in the theorem are with respect to
$\min_{s,m}\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}})
\rightarrow \infty$. The implications of the asymptotics are best
explored by the way of example. For example, if
$\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}$ is scalar for all sensors at all
times, $\bR_{\zeta_{m}^{s}\zeta_{m}^{s}} = {\sigma^2}_{m}^{s}$, then
$\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}) =
{\sigma^2}_{m}^{s}$. And the asymptotic requirement becomes for the
measurement noise variance to go to infinity for all sensors at all
times. Or, equivalently, for all measurements to become utterly
uninformative. If, on the other hand,
$\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}$ is $2\times 2$ with equal
component variances, for all sensors at all times:
\begin{align}
\bR_{\zeta_{m}^{s}\zeta_{m}^{s}} = {\sigma^2}_{m}^{s}
\begin{pmatrix} 1 & \rho_{m}^{s} \\
\rho_{m}^{s} & 1
\end{pmatrix}
\end{align}
then $\lambda_{\min}(\bR_{\zeta_{m}^{s}\zeta_{m}^{s}}) =
{\sigma^2}_{m}^{s}(1-|\rho_{m}^{s}|)$. Thus the asymptotic
requirement is for measurement components not to be absolutely
(positively or negatively) correlated ($|\rho_{m}^{s}| \neq 1,
\forall m,s$), and to have asymptotically large variance.

This leads us to the conclusion that the algorithm we described is
asymptotically optimal under regularity conditions. The asymptotics
are with respect to increasing variance of reasonably correlated
measurement noises. The regularity conditions ensure smoothness of
measurement and transition functions (existence of the EKF
approximation) and the proper operation of the EKS.


==> section7.tex <==
\section{Numerical Experiments} \label{Sec:7}

\noindent In our simulations we consider a two-dimensional scenario
with a single target that makes a clockwise coordinated turn of
radius $500m$ with a constant speed $200km/h$. It starts in
y-direction with initial position $[-500m,500m]$ and is tracked for
$40$ seconds.

The target motion is  modeled in the filters by the nearly
coordinated turn model~\cite{Bar-Shalom2001} with unknown constant
turn rate and cartesian velocity. The state of the target is given
as $x_k=[p_k^x,p_k^y, v_k^x,v_k^y, \omega_k]^T $, where $p,v$ and
$\omega$ denote the position, velocity and turn rate respectively.
The dynamic model for the coordinated turn model is
\begin{equation*}
X_{k+1}=
\begin{pmatrix}
1 & 0 & \frac{\sin(\omega_k)}{\omega_k}    & \frac{\cos(\omega_k)-1}{\omega_k}    & 0 \\
0 & 1 & \frac{1- \cos(\omega_k)}{\omega_k} & \frac{\sin(\omega_k)}{\omega_k}      & 0 \\
0 & 0 & \cos(\omega_k)                     & -\sin(\omega_k)                      & 0 \\
0 & 0 & \sin(\omega_k)                     & \cos(\omega_k)                       & 0 \\
0 & 0 & 0                                           & 0 & 1
\end{pmatrix}
X_k + \vartheta_{k+1}
\end{equation*}
where $\vartheta_{k+1}$ is Gaussian process noise,
$\vartheta_{k+1}\sim \mathcal{N} (0,\bV_{k+1})$,
$\bV_{k+1}=\diag([30^2, 30^2, 10^2,10^2,0.1^2 ])$, the sampling
period is $1$ second. We assume that the filter initially knows
little about the state of the target and therefore it is initialized
with the state value $\mu_{X_0} = [0,0,0,0,0]^T$ and a large
covariance $\bR_{X_0 X_0}= \diag([1000^2,1000^2,30^2,30^2,0.1^2])$.

There are three sensors S1, S2 and S3 sending bearing-only
measurements of the target to a common fusion centre. The sensor
locations are $[S_1^x,S_1^y]=[-200,0]$, $[S_2^x,S_2^y]=[200,0]$,
$[S_3^x,S_3^y]=[-750,750]$ and the bearings-only measurement
function is
\begin{equation}
\mathit{h}_k^j(x_k)=\arctan(\frac{p_k^y-S_j^y}{p_k^x-S_j^x}) \
j=1,2,3
\end{equation}
The measurements from the sensors are corrupted with additive
independent Gaussian noises with zero mean and standard deviation
$\sigma_s=0.05$. An OOSM arrives at the fusion centre from a given
sensor with probability $p_{osm}$ and delay $d$. The delay $d$ is
uniformly distributed in the interval $[0,5]$. The probability
$p_{osm}$ that an OOSM reaches the fusion centre at all is set to
$0.7$.


\begin{figure}[t]
\centering \subfigure[N=2000]{ \label{fig:RMS:2000}
\includegraphics[width = 8cm]{RMS_N2000_Ntr5000_Th6.eps}}
 \subfigure[N=5000]{\label{fig:RMS:5000} %% label for second subfigure
\includegraphics[width = 8cm]{RMS_N5000_Ntr5000_Th6.eps}}
\caption{Tracking performance of the particle filters as a function
of
  time using RMS error as a performance metric. The curves show the
  means of 5000 Monte-Carlo trials. (a) Filters use 2000 particles;
  (b) Filters use 5000 particles.}
\label{fig:RMS} %% label for entire figure*
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[width = 8cm]{ex2_ErrorBar_N5000_Ntr5000_Th6.eps}
\caption{Errorbars showing the variation of position RMS for
  \textit{SEPF-EKS}, \textit{PF-GS} and \textit{PF-SEL}, when they use 5000
  particles. The box has lines at the lower quartile, median(red line), and upper quartile values. Outliers (red '+') are values beyond the range of 5 times the interquartile range from the ends of the box.}
  %Top panel: Storage Efficient Particle Filter (PFEKS); middle panel: OOSM-GARP particle filter (PF-GS);bottom panel: Selective processing particle filter using the mutualinformation metric.
\label{fig:Errorbar} %% label for entire figure*
\end{figure}
\subsection {Benchmarked Filters}
\noindent We have implemented five different particle filters, all
based on the Sampling Importance Resampling (SIR) filtering
paradigm~\cite{Gordon1993}. The prior distribution is used as the
importance function. The filters were implemented in Matlab and the
code was highly optimized.

\textit{PFall}: collects all measurements from all active sensors
(no OOSMs). This is an idealized filter that provides a performance
benchmark.

\textit{PFmis}: discards all OOSMs and therefore only processes the
measurements with zero delay.

\textit{SEPF-EKS}: Storage efficient particle filter using EKS
smoothing as described in~\cite{Orguner2008} and described in
Algorithm~\ref{alg:SEPF-EKS}.

\textit{PF-GS}: The OOSM-GARP algorithm described in
Algorithm~\ref{alg:ProcessOOSM-GARP}.

\textit{PF-SEL}: Selective OOSM processing based on the proposed
framework and described in Algorithm~\ref{alg:PROPOSED}.

We use the root mean-squared (RMS) position error to compare the
performances of particle filters. Let $({p_k^x},{p_k^y})$ and
$(\hat{p}_{k,i}^{x},\hat{p}_{k,i}^{y})$ denote the true and
estimated target positions at time step $k$ for the $i$-th of $M$
Monte-Carlo runs. The RMS position error at $k$ is calculated as
\begin{align}
\RMS_k = \sqrt{\frac{1}{M} \sum_{i=1}^{M}
(\hat{p}_{k,i}^{x}-{p_k^x})^2 + (\hat{p}_{k,i}^{y}-{p_k^y})^2 }
\end{align}

\subsection{Results and Discussion}

\noindent In our first experiment we fix the computational cost
$C_{\ave} = 0.6$. We thus allow $0.6$ sweeps of the SEPF-EKS
algorithm to be performed on average per filtering step. Over an
extended period of time of sufficiently large length $L$ this leads
to an additional OOSM processing overhead of $\sim 0.6 L C_{EKS}$
where $C_{EKS}$ is the cost of one sweep of the SEPF-EKS algorithm.
If we do not apply the proposed procedure and process all the
available OOSMs this cost in our application scenario is around
$\sim 1.4 \ldots 1.8 L C_{EKS}$. This implies that we process only
approximately $43 \ldots 33 \%$ of all measurements.

In Fig.~\ref{fig:RMS}, we plot the respective RMS position
performance for the tracking period of $40s$ for the algorithms with
these settings. Corresponding error-bar plots of the RMS performance
are shown in Fig.~\ref{fig:Errorbar}. The actual number of
individual OOSMs to be processed by the SEPF-EKS after the first
threshold $\gamma_k$ measured in our experiment is $40.04\%$ and
$39.97\%$ with $2000$ and $5000$ particles respectively. After the
second threshold $\nu = 1/40$ the number of most informative OOSMs
processed by rerunning the particle filter is $1.57\%$ and $1.44\%$
with $2000$ and $5000$ particles respectively.

Fig.~\ref{fig:RMS} indicates that despite processing only a
relatively small fraction of the OOSMs, the proposed algorithm
performs almost as well as the much more complex OOSM-GARP algorithm
(\textit{PF-GS}). The calculation of the selection criterion has
minimal overhead, so discarding the uninformative measurements
results in significant computational savings. Thus the proposed
filter is more computationally efficient than the SEPF-EKS filter
and yet, as can be seen from Fig.~\ref{fig:RMS}, it has better RMS
performance. Fig.~\ref{fig:Errorbar} indicates that the performance
of SEPF-EKS is not as stable as that of \textit{PF-GS} and
\textit{PF-SEL}. In the proposed algorithm the increased robustness
and performance stability is achieved by using the second threshold
to detect situations when reweighing induces sample degeneracy
problems.


In our next experiment we study the computational complexity versus
accuracy trade-off for the proposed algorithm. We illustrate this by
varying the computational complexity of the proposed algorithm by
adjusting $C_{\ave}$ and plot the RMS vs. complexity curve measured
in MATLAB. We use the following values to control the OOSM
processing overhead: $C_{\ave} = \{0, 0.1, 0.2, 0.4, 0.5, 0.6, 0.78,
1, 1.3, 2\}$, $\gamma_2= 1/40$. These results are reported in
Fig.~\ref{fig:RMS_Complexity}. In this figure we show the
relationship between complexity and performance for the proposed
algorithm with ten values of $C_{\ave}$ and results of 10
simulations for other algorithms. Each simulation involves 1000
Monte Carlo runs. We compare the performance of all particle filters
when they use $2000$ and $5000$ particles. When the thresholds are
chosen so that the proposed filter has the same computational
complexity as SEPF-EKS, it achieves significantly better tracking
performance. Alternatively, for the same fixed RMS error
performance, the selective processing algorithm reduces the
computation time by up to $50\%$. Also we can see that by using the
appropriate setting of $C_{\ave}$ we can achieve the required
trade-off between the average computational load or power supply
consumption and the tracking performance. This inherent flexibility
of the algorithm based on the proposed framework is a novel property
not observed in the algorithms previously reported in the
literature.

\begin{figure*}[t]
\centering \subfigure[$N=2000$, $t=10$]{
\label{fig:RMS_Complexity:N2000_t10}
\includegraphics[width = 8cm]{RMS_Complexity_N2000_Ntr5000_T10.eps}}
 \subfigure[$N=5000$, $t=10$]{\label{fig:RMS_Complexity:N5000_t10} %% label for second subfigure
\includegraphics[width = 8cm]{RMS_Complexity_N5000_Ntr5000_T10.eps}}
 \subfigure[$N=2000$, $t=20$]{\label{fig:RMS_Complexity:N2000_t20} %% label for second subfigure
\includegraphics[width = 8cm]{RMS_Complexity_N2000_Ntr5000_T20.eps}}
\centering \subfigure[$N=5000$, $t=20$]{
\label{fig:RMS_Complexity:N5000_t20}
\includegraphics[width = 8cm]{RMS_Complexity_N5000_Ntr5000_T20.eps}}
 \subfigure[$N=2000$, $t=30$]{\label{fig:RMS_Complexity:N2000_t30} %% label for second subfigure
\includegraphics[width = 8cm]{RMS_Complexity_N2000_Ntr5000_T30.eps}}
 \subfigure[$N=5000$, $t=30$]{\label{fig:RMS_Complexity:N5000_t30} %% label for second subfigure
\includegraphics[width = 8cm]{RMS_Complexity_N5000_Ntr5000_T30.eps}}
\caption{RMS vs Complexity from $10$ simulations with different
$C_{\ave}$. Each simulation shows the average of $1000$ MC runs.We
select three timesteps, $t=10,20,30$ for filters with $2000$ and
$5000$ particles. The complexity is measured by running time for
tracking $40$s of each filter. The results are run on a Dell laptop
with Genuine Intel(R) CPU T2400 1.83GHz, 0.99GB RAM and Win-XP OS.}
\label{fig:RMS_Complexity} %% label for entire figure*
\end{figure*}

